DNN Memory Footprint Reduction via Post-Training Intra-Layer Multi-Precision Quantization

The imperative to deploy Deep Neural Network (DNN) models on resource-constrained edge devices, spurred by privacy concerns, has become increasingly apparent. To facilitate the transition from cloud to edge computing, this paper introduces a technique that effectively reduces the memory footprint of DNNs, accommodating the limitations of resource-constrained edge devices while preserving model accuracy. Our proposed technique, named Post-Training Intra-Layer Multi-Precision Quantization (PTILMPQ), employs a post-training quantization approach, eliminating the need for extensive training data. By estimating the importance of layers and channels within the network, the proposed method enables precise bit allocation throughout the quantization process. Experimental results demonstrate that PTILMPQ offers a promising solution for deploying DNNs on edge devices with restricted memory resources. For instance, in the case of ResNet50, it achieves an accuracy of 74.57\% with a memory footprint of 9.5 MB, representing a 25.49\% reduction compared to previous similar methods, with only a minor 1.08\% decrease in accuracy.

==> relate.tex <==
% \section{Background and Related Work}
\section{Related Work}
\label{sec:related}
% Compression is one of the common methods to reduce the size of the NN while maintaining its accuracy. Compression methods have various categories. One type of their classification is \cite{choudhary2020comprehensive}: pruning methods \cite{li2017pruning, theis2018faster}, knowledge distillation \cite{hinton2015distilling, yim2017gift}, low-rank factorization \cite{lowrank,povey2018semi} and quantization \cite{zhou2017balanced,krishnamoorthi2018quantizing, nagel2019data}. 


In this paper, the focus is on the quantization method, and in this section, various quantization are discussed.

% NN quantization, by mapping weight values and activation functions or only by mapping weight values from 32-bit floating point to integers, while maintaining the accuracy of the NN, reduces the size of the NN to an acceptable level. The main idea of quantization operation is not new and was proposed in the articles \cite{fiesler1990weight, balzer1991weight} in 1990. On the other hand, DNNs have many parameters, which can dramatically reduce the size of the NN and the volume of calculations by using quantization operations. First, the quantization techniques used in this article are reviewed. Then the previous works related to the proposed method are reviewed.

% \subsection{Background}
% Quantization is classified into two categories based on quantization levels, uniform and non-uniform quantization. In uniform quantization, floating point numbers are mapped to integers with the same distance \cite{baskin2021uniq, nagel2019data}. On the other hand, if the quantization levels are not uniform and have an unequal distance from each other, it is called non-uniform quantization \cite{li2019additive, jeon2020biqgemm}. Figure \ref{fig:uniform} shows uniform and non-uniform quantization. In Figure \ref{fig:uniform}, the horizontal axis is the real numbers and the vertical axis is the quantization levels. In figure \ref{fig:uniform}.a, there are lines with unequal distance from each other (non-uniform quantization). In figure \ref{fig:uniform}.b, these lines are at the same distance from each other (non-uniform quantization). The accuracy of the NN in non-uniform quantization may be higher than in uniform quantization. Because in non-uniform quantization, by focusing more on important value areas or finding appropriate dynamic ranges, distributions can be depicted better. Because in non-uniform quantization, by more focusing on important areas or finding appropriate dynamic ranges, distributions can be depicted better. But implementing non-uniform quantization on common hardware such as CPU and GPU is difficult. In contrast, the implementation of uniform quantization is done simply. Therefore, uniform quantization is more important. 

% % \begin{figure}
% %     \centering
% %     \includegraphics[width=.8\columnwidth]{Figs2/uniform, nonuniformv13.pdf}
% %     \caption{illustration of two types of quantization: non-uniform quantization and Uniform quantization. Input weights are shown on the x-axis and quantization levels on the y-axis. Quantization levels are the same in Uniform quantization, while quantization levels are differ in Non-Uniform quantization.  }
% %     \label{fig:uniform}
% % \end{figure}

% In the quantization operation, if the maximum and minimum value of the interval are relative to each other, it is called symmetric quantization \cite{https://doi.org/10.48550/arxiv.1807.00301}, and if the maximum and minimum are not relative to each other, it is called asymmetric quantization. Figure \ref{fig:symmetric} shows these two quantization. 

% % \begin{figure}
% %     \centering
% %     \includegraphics[width=.8\columnwidth]{Figs2/symmetric vs asymmetricV7.pdf}
% %     \caption{symmetric and asymmetric quantization.}
% %     \label{fig:symmetric}
% % \end{figure}

% Where the r axis represents real numbers in floating point format, the Q axis represents numbers corresponding to integer format. In Figure \ref{fig:symmetric}.a, the maximum and minimum are related to each other, but in Figure \ref{fig:symmetric}.b, the maximum and minimum have no relationship with each other. Symmetric quantization has a simpler implementation and lower computational cost in the inference process than asymmetric quantization due to the existence of symmetry in the cutoff interval \cite{https://doi.org/10.48550/arxiv.2004.09602}. In cases where the data interval is skewed and there is no symmetry, asymmetric quantization will perform better \cite{https://doi.org/10.48550/arxiv.2103.13630}.

% Typically, in NNs, weights and activation functions are stored with 32-bit floating-point precision. By using the quantization technique, both or only the weights can be stored with 16-bit, 8-bit, 4-bit and even 2-bit integer precision. In quantization with low precision, due to the reduction in the number of bits, the accuracy of the NN decreases. One of these approaches is to retrain the DNN after performing the quantization operation, which requires access to the training data, which results in high processing overhead for retraining. Methods that use this approach to compensate for lost accuracy fall under the category of Quantization Aware Training and benefit from high accuracy. Although the accuracy of the NN using QAT will be higher than PTQ. PTQ is superior to QAT in terms of privacy and security, and it will be faster and less expensive to train because it does not require retraining. Figure \ref{fig:ptq} shows an overview of the QAT and PTQ multiplication process.

% % \begin{figure}
% %     \centering
% %     \includegraphics[width=.8\columnwidth]{Figs2/ptq and qat flow ENGv13.pdf}
% %     \caption{Quantization Aware Training (QAT) and Post Training Quantization (PTQ).}
% %     \label{fig:ptq}
% % \end{figure}

% In Figure \ref{fig:ptq}.a, the training dataset is used to retrain the quantized NN and compensate for the lost accuracy, which makes the accuracy of this technique high. But in Figure \ref{fig:ptq}.b, using the calibration dataset, the initialization operation is done to the activation functions, and then the quantization is done. Hence, due to the elimination of the retraining operation, the computational overhead is reduced, but the accuracy of the NN using this technique is lower in most cases compared to the QAT technique. If in the quantization operation, different bit precision use for the layers or channels of the NN, it is called mixed precision quantization. But if all layers or channels quantize with fixed bit precision, it is called single precision quantization. In mixed precision quantization, due to the possibility of specifying different bit precision for each layer or channel, more compression can be done on the NN model.

% \subsection{Related works}
% Due to the importance of access or lack of access to training dataset, as well as doing or not doing the re-training process after the quantization operation, placing a paper in the PTQ or QAT category is of particular importance. 

% In the PTQ category, techniques are presented to compensate or reduce the lost accuracy. When quantizing an NN based on the PTQ technique, the accuracy of the NN decreases due to the lack of retraining process. 
% \cite{}[ZEROQ paper] uses the NN weights simulation technique to reduce the lost accuracy and compensate for it due to quantization. In this paper, synthetic data are generated similar to real data, and the lost accuracy of the NN is compensated by retraining the NN with these data. Noted that this technique will not be a problem from the point of view of security and privacy because it does not require training data and performs the retraining process without access to the training dataset. But this technique also performs the retraining process in a way, and it will result in a lot of overhead for creating artificial data and the retraining process. [PWLQ article] \cite{} uses the technique of non-overlapping regions to avoid reducing the accuracy of the NN. Usually, in the NNs, the distribution of weights is bell-shaped. Therefore, the authors define breaking points on the distribution of NN weights. These breakpoints are calculated based on the quantization error. Based on these points, the weight distribution range is divided into non-overlapping areas. The weights of the NN, which are floating point precision, are placed in one of the defined intervals according to their value, and unlike the uniform quantization where all the weights are placed in the same interval. In this technique, each weight is quantized based on the area in which it is placed. But in this paper, the precision of quantization is the same and all the weights are quantized by a fixed number (Single precision quantization). Therefore, it does not benefit from the advantage of mixed precision, and in cases where there is a limitation of storage memory, this technique may become ineffective. In the proposed method, we solve this problem by using the mixed precision technique and determining the importance for each layer.




% ZEROQ and PWLQ, are included in the PTQ category and use two different techniques to avoid reducing the accuracy of the NN.
% Also, for the mixed precision technique, HAWQV2 and AdaQuant have provided two different techniques to separate the layers, which are reviewed below.




% (Figure \ref{fig:distribution} shows how the weights are distributed).
% Therefore, performing the quantization operation based on this technique has less error than the uniform quantization method.
% In the proposed method, this technique is used to divide the overall weight distribution interval into smaller non-overlapping intervals. 
% Because in this technique, without performing the retraining process, the accuracy of the NN increases significantly.
% and it is possible to map floating point numbers to integers with 8-bit, 4-bit and even 2-bit without accessing the training data and producing artificial data with acceptable accuracy.
% HAWQV1, which uses the mixed precision technique, considers a different bit precision for each layer. In this article, to determine the importance of each layer, the value of Hessian eigenvalues of each layer is calculated and based on that, the importance of the layers is determined. Each layer that is included in the category of important layers is assigned a high bit precision to perform quantization operations. This paper is included in the QAT category because after performing the quantization operation, the NN model is trained using the training dataset in the retraining process and its lost accuracy is compensated. Therefore, this technique requires access to the training dataset. The authors of QWP suggest quantizing the activation functions to 8-bit to increase the speed and also reduce the memory consumption in the inference process, and they claim that this will increase the speed of the inference process by 2-3 times because both the memory consumption and calculations are reduced. But PTQ quantization is only done with 8-bit precision. The DFQ paper performs quantization without performing a retraining operation. The authors of this paper claim that channel-wise quantization works better in models such as MobileNetV2, because the distribution of weights of each channel differs greatly from the other. They also believe that the quantization error may cause a bias error on the corresponding outputs. Therefore, they suggest a technique to correct the created error. This technique works well for quantization with 8-bit precision and the decrease in accuracy is insignificant, but in quantization with 4-bit precision, it causes a sharp decrease in the NN accuracy.

% In the HMQ article, for hardware-friendly mixed precision quantization operations, blocks are defined that determine the quantization precision for each block and perform quantization operations based on them. However, in this method, after performing the quantization operation, due to the decrease in the accuracy of the NN, the training operation is performed again.

% The authors of the SSBD paper propose a new technique for weight factorization. Using this technique, neural network channels are equalized, and outliers are removed. Hence, the NN is more tolerant to the quantization operation.

% In the paper AdaRound, a new mechanism for rounding the value of the NN weights is presented. By using the Taylor series expansion on the Loss function, the rounding operation is presented as a binary optimization problem and this operation is performed layer by layer. The AdaQuant paper, which uses the mixed precision technique, has presented another technique to determine the importance of each layer. In this paper, an integer-programming (IP) formula is defined, which is calculated for the purpose of loss degradation, and based on which the importance of each layer is determined. Also, for each layer, the value of the quantization error is calculated and based on that, the precision of quantization is determined. But this technique specifies the bit precision of quantization only at the level of NN layers and is not effective in performing quantization operations with 2-bit precision.

% The authors of the DDQ paper claim to present a completely different method for learning NN parameters and quantization. In this paper, an algorithm for automatic learning of quantization policies such as quantization levels and quantization precision is defined. Using this technique, it is possible to quantize small models like MobileNetV2.

% According to the PTQ and QAT quantization concepts, previous works are separated in Table \ref{tab:compare}.
% Also, each of them has been distinguished from each other due to the use of mixed precision technique. The proposed method is placed in the PTQ category. In the proposed method, the calibration dataset is used to calibrate the activation functions.


% \begin{table}[tb!]
%     \centering
%         \caption{Identification whether the methods post training quantization or quantization aware training, and which methods use mixed-precision.}
%     \begin{tabular}{c||c|c||c|c}
%     \hline
%         method & \multicolumn{2}{c||}{PTQ VS. QAT} & \multicolumn{2}{c}{Single VS. Mixed precision} \\
%         \hline
%          & PTQ & QAT & Single-precision & Mixed-precision\\
%          \hline
%          ZEROQ \cite{cai2020zeroq} & \cmark &  & & \cmark \\
%          PWLQ \cite{fang2020post} & \cmark &  & \cmark &\\
%          HAWQV2 \cite{dong2019hawq} & & \cmark & & \cmark  \\
%          QWP \cite{krishnamoorthi2018quantizing} & \cmark &  & \cmark & \\
%          DFQ \cite{nagel2019data} & \cmark &  & \cmark &\\
%          HMQ \cite{habi2020hmq} & & \cmark & & \cmark \\
%          SSBD \cite{meller2019same} & & \cmark &  \cmark & \\
%          AdaRound \cite{nagel2020up} & \cmark &  & & \cmark\\
%          AdaQuant \cite{hubara2020improving} & \cmark &  & & \cmark\\
%          DDQ \cite{zhang2021differentiable} & & \cmark & & \cmark \\
%          \rowcolor{mycolor}
%          Ours & \cmark &  & & \cmark \\
%     \hline
%     \end{tabular}
%  		\vspace{-0.1in}
%     \label{tab:compare}
% \end{table}
